EASI Drugs in the Streets of Colombia: Modeling Heterogeneous and Endogenous Drug Preferences

The response of illicit drug consumers to policy changes like legalization is mediated by demand behavior. Since individual drug use is driven by many unobservable factors, accounting for unobserved heterogeneity becomes crucial for designing targeted policies. This paper introduces a finite Gaussian mixture of EASI demand systems to estimate joint demand for marijuana, cocaine, and basuco (a low-purity cocaine paste) in Colombia, accounting for corner solutions and endogenous prices. Our method classifies users into two groups with distinct preferences over consumption: "soft" and "hard" users. Nationally representative survey estimates find drugs are unit-elastic, with marijuana and cocaine complementary. International marijuana legalization episodes along with Colombia's low marijuana production cost suggest legalization is likely to drive prices down significantly. Legalization counterfactuals under the most likely scenario of a 50\% marijuana price decrease reveal \$363/year welfare gains for consumers, \$120M in governement revenue, and \$127M dealer losses.

==> Floats/Density_ProfitChange_Scenario50.tex <==
\begin{figure}
    \centering
    \caption{Density plot of changes in drug dealer marijuana profits following a price change in marijuana implied by EASI system estimates from ``safe'' cluster}
    \label{Fig:Density_ProfitChange_Scenario50}
    \resizebox{1\textwidth}{!}{%
    \begin{threeparttable}
         \centering
         \includegraphics[width = \textwidth, page = 2]{Figures/ProfitChange_Bayes_Homogeneous_Mixture_PriceChange_0.5.pdf}
    \begin{tablenotes}
    \item \small{\textbf{Notes:} Full posterior density over the change in total marijuana profits given in millions of 2019 USD\$ after a 50\% decrease in the price of marijuana and complete access to dealers following legalization of marijuana. Dealers are assumed to keep only 34\% of the legal market of marijuana post-legalization and pay 2.1 cents per gram produced. Dashed line represents median of chains, dotted line provides the 95\% HPD for each parameter, and a solid line at 0 is drawn for reference. Single chain run keeping 10000 draws after a burn-in window of 5000 iterations, discarding every 10 draws.}
    \end{tablenotes}
    \end{threeparttable}
    }
\end{figure}
